On Robustness to $k$-wise Independence of Optimal Bayesian Mechanisms

This paper reexamines the classic problem of revenue maximization in single-item auctions with $n$ buyers under the lens of the robust optimization framework. The celebrated Myerson's mechanism is the format that maximizes the seller's revenue under the prior distribution, which is mutually independent across all $n$ buyers. As argued in a recent line of work (Caragiannis et al. 22), (Dughmi et al. 24), mutual independence is a strong assumption that is extremely hard to verify statistically, thus it is important to relax the assumption. While optimal under mutual independent prior, we find that Myerson's mechanism may lose almost all of its revenue when the independence assumption is relaxed to pairwise independence, i.e., Myerson's mechanism is not pairwise-robust. The mechanism regains robustness when the prior is assumed to be 3-wise independent. In contrast, we show that second-price auctions with anonymous reserve, including optimal auctions under i.i.d. priors, lose at most a constant fraction of their revenues on any regular pairwise independent prior. Our findings draw a comprehensive picture of robustness to $k$-wise independence in single-item auction settings.

==> sec/idencopy.tex <==
We consider in this section a special case of identical marginal prior distributions $\disti=\dist$ for all $i\in[n]$. Then Myerson auction is the same as the second price auction with the monopoly reserve price $\mr$ (the virtual value $\virt(\mr)=0$), when the prior $\dist$ is a regular distribution. It turns out that in this case, the Myerson auction is pairwise-robust even for the case of non-regular prior $\dist$.



%In this section, we prove the following theorem:
%\nick{Are we assuming in this section that prior $\dist$ is regular? As far as I remember you did not need regularity, right?}
%\nick{I think it might be easier to write approximation constants $c$ as $c>1$ rather than $c<1$.}
\begin{theorem}
\label{thm: myersoniid}
Myerson auction is pairwise-robust for any identical marginals $\dist$ with a constant $c< 2.63$.
\end{theorem}
\begin{proof}
%\nick{Did you know that it is okay to have lemmas with proofs inside the proof of a theorem?}
% \begin{theorem}
% \label{thm: myersoniid}
% Myerson auction is pairwise-robust for identical distributions, where it degenerates to second price auction with reserve. Moreover, the constant $c$ is larger than $\frac{1}{2.63}$.
% \end{theorem}
%\nick{Again you scramble the order of sentences. Once you introduce opt, you want to say that we want to give an upper bound on it similar to ex-ante relaxation. Then you introduce all necessary notations and present the lemma.

%\nick{IMPORTANT CHANGE: $\dist$ is the distribution after ironing, as well as $\Quan(\cdot)$.}
We first prove the case for regular distribution, the case of non-regular distribution is a direct corollary.
We denote the revenue of the optimal Myerson auction under mutually independent distribution $\distind$ as $\opt$ and derive an upper bound on $\opt$ similar to a widely used Ex-ante relaxation. Let $\ww$ be a threshold such that $\Quan(\ww) = \frac{1}{n}$ (if $\ww$ does not exist, we define $\ww\eqdef \sup\{\val~|~\Quan(\val)\ge \frac{1}{n}\}$), then the Ex-ante relaxation gives an upper bound $\opt\leq \ww$. 
% If there exists some value $\valo$ such that $\Quan(\valo) = \frac{1}{n}$, then the classical Ex-ante relaxation gives an upper bound $\opt\leq \valo$. 
%We assume that $\dist$ is already ironed, i.e., its quantile $\Quan(\val)$ corresponds to the distribution with the ironed revenue curve.
%\wzq{VERY IMPORTANT CHANGE:}
% Let $\ww\eqdef \sup\{\val~|~\Quan(\val)\geq \frac{1}{n}\}$. 
The following lemma extends the Ex-ante relaxation bound to a broader range of values $\ww$.
% We can use the following lemma which can be regarded as a general version of ex ante relaxation to lower bound the ratio between such $\val$ and $\opt$.
%\nick{Bad choice of notation $\val$ in the lemma: we use $\val$ as generic variable, often with $\val\sim\dist$, but here it is a fixed quantity.}
\begin{lemma}[Ex-ante relaxation]
\label{lem: exante}
%Denote the optimal reserve as $\mr$. 
Assuming the value distribution $\dist$ is regular.
For any $\valo\in [\mr,w)$ when $\mr\le\ww$, and $\valo=\mr$ when $\ww<\mr$ we have  
\begin{equation}
    \valo \geq \frac{\opt}{n\cdot\Quan(\valo)}.
\end{equation}
% Denote the optimal reserve as $\reserve^*$. Then
% $\forall \val$ such that $\reserve^*\leq \val\leq \ww$, or $\ww\leq \val = \reserve^*$ we have
% \begin{equation}
%     \val \geq \frac{\opt}{n\cdot\Quan\left (\val\right )}.
% \end{equation}
\end{lemma}
\begin{proof}
%\wzq{I checked that the current proof only holds for regular distribution. So we don't need to use the ironed virtual value function}
%\wzq{But is there any alternative bound like ex-ante relaxation for irregular distribution?}

Let $\virt \left(\cdot\right )$ be the virtual value function.
We fix the joint prior distribution to be $\distind$.  
Let the random variable $\maxvirt\eqdef \max_{i\in[n]}\virt(\vali)$ for $\vals\sim\distind$ be the maximum virtual value. 
Then
\begin{multline*}
    \opt = \Ex{\maxvirt^{+}}=
    \Ex{\min\{\maxvirt^{+}, \virt\left (\valo\right )\}} +\Ex{\left (\maxvirt - \virt\left (\valo\right )\right )^{+}}\\
    \le \virt\left (\valo\right ) + n\cdot \Ex[\val]{\left(\virt\left (\val\right ) - \virt\left(\valo\right )\right )^{+}}
    = \virt\left(\valo\right ) + n\cdot\Quan\left(\valo\right )\cdot \left(\valo - \virt\left(\valo\right )\right )\\
    = n\cdot\Quan\left(\valo\right )\valo - \left(n\cdot\Quan\left (\valo\right ) - 1\right )\virt\left (\valo\right )
    \leq n\cdot\Quan\left(\valo\right )\valo,
\end{multline*}
%\nick{In a chain of nontrivial inequalities, usually it is a good idea to give some explanations about each step.}
where the first equality holds as the auction's expected revenue is equal to the expected virtual welfare; the second equality holds as $\virt(\valo)\ge 0$ (recall that virtual function is weakly increasing for a regular distribution and $\valo\ge\mr$); the first inequality is due to the facts that $\min\{\maxvirt^{+}, \virt\left (\valo\right )\}\le\virt\left(\valo\right)$ and that $\max_{i\in[n]}(a_i-c)^{+}\le\sum_{i\in[n]}(a_i-c)^+$ for any $a_i\in\R$ and $c\in\R$; the third equality holds as $\Ex[\val]{\left(\virt\left (\val\right ) - \virt\left(\valo\right )\right )^{+}}=
\Ex[\val]{\virt\left(\val\right )\cdot\ind{\val\ge\valo}}-
\virt\left(\valo\right)\cdot\Quan(\valo)$ and $\Ex[\val]{\virt\left(\val\right )\cdot\ind{\val\ge\valo}}=\valo\cdot\Quan\left(\valo\right)$ is the revenue of selling the item to a single agent at the price $\valo$; the final inequality is due to the fact that $\Quan(\valo)\le\frac{1}{n}$.
\end{proof}



We are now ready to finish the proof of Theorem~\ref{thm: myersoniid}.
The first useful observation is that for each $\valo < \ww$ (i.e., $\Quan(\valo)> \frac{1}{n}$) there is a positive probability that at least two bidders have a value larger than $\valo$ by Lemma~\ref{lem: ziyong}.
% \nick{How is the previous sentence related to ex-ante relaxation?}
% \wzq{I don't know, I think it is very different from the ex-ante relaxation. The reason for this sentence is that the sum of the probability is larger than 1, there must be some case that at least two bidders' value is larger than $\valo$.}
% % \paragraph{Proof of Theorem \ref{thm: myersoniid}} 
% \nick{$k$ is usually reserved for integers.}
We also need to consider the relation between $\mr$ and $\ww$. To this end, let us define $\kk\eqdef \frac{1}{n\cdot\Quan\left (\mr\right )}$. We consider two cases. 
First, if $\kk \ge 1$, i.e. $\mr \geq \ww$. Then 
\begin{equation*}
\Rev\left (\dists, \gM\right ) \geq \frac{\kk\cdot \reserve^*}{\kk + 1} \geq \frac{\kk^2\cdot \opt}{\kk + 1} \geq \frac{1}{2}\cdot \opt,
\end{equation*}
where the first inequality holds by Lemma~\ref{lem: wine}: the probability that item is sold is at least $\frac{\kk}{\kk + 1}$ at a price at least $\mr$; the second inequality holds by Lemma~\ref{lem: exante} for $\valo = \mr$; the last inequality is due to $\kk \ge 1$.

Second, if $\kk< 1$. 
In this case, we directly analyse the payment in the Myerson auction. When the payment is realized, we apply Lemma~\ref{lem: exante} to give a lower bound for the ratio between the payment and the optimal revenue. 
Specifically, let $\Payment=\sum_{i\in[n]}\payi(\vals)$ be a random variable denoting the payment of Myerson auction for $\vals\sim\dists$.
Since Lemma~\ref{lem: exante} is valid only for $\valo \in  [\reserve^*, \ww]$, we denote $\Payment'\eqdef\min\{\Payment, \ww\}$. Then by Lemma~\ref{lem: exante}
applied to each realization of $\Payment'\in[\mr,w]$
% Suppose the payment of Myerson auction under $\distpi$ is a random variable $\Payment$. 
% Note that the condition of lemma \ref{lem: exante} requires that $\reserve^*\leq v\leq w$.
% If $P \geq w$, we can simply regard the payment as $w$ when using the lemma.
% Denote $\Payment' = \min\{\Payment, \ww\}$.
% Then according to lemma \ref{lem: exante} we have
\begin{equation*}
\label{eq: thm1}
\Ex[\vals\sim\dists]{\Rev(\vals)} = \Ex{\Payment} \ge \Ex{\Payment'}\geq \Ex{\frac{\ind{\Payment'\ge\mr}}{n\cdot\Quan\left (\Payment'\right )}}\cdot \opt.
\end{equation*}
where the first inequality holds as $\Payment\geq \Payment'$; the second inequality is due to Lemma~\ref{lem: exante}.
This allows us to write the following lower bound on the ratio between the revenue under pairwise independent distribution and $\opt$. 

\begin{multline}
\frac{\Ex[\vals\sim\dists]{\Rev(\vals)}}{\opt} \ge \Ex{\frac{\ind{\Payment'\ge\mr}}{n\cdot\Quan\left (\Payment'\right )}}
 = \kk\cdot \prob{\frac{1}{n\cdot\Quan\left (\Payment'\right )}\geq \kk} + \int_\kk^1\prob{\frac{1}{n\cdot\Quan\left (\Payment'\right )}\geq u}\d u \\
 = \kk\cdot \prob{\Payment' \geq \reserve^* = \Quan^{-1}\left(\frac{1}{n\cdot \kk}\right)}+ \int_\kk^1\prob{\Payment'\geq \Quan^{-1}\left(\frac{1}{n\cdot u}\right)}\d u,
 \label{eq: iidratio}
\end{multline}
where the first equality holds as (a) $\Ex{Y}=\int_{0}^{\infty}\Prx{Y\ge u}\d u$ for any random variable $Y\ge 0$ and (b) $Y\in[\kk,1]\cup\{0\}$, because
$\mr\leq \Payment'\leq w$ and $\kk\leq \frac{1}{n\cdot\Quan\left (\Payment'\right )}\leq 1$.
Now, the event that $\Payment' \ge \mr$ in \eqref{eq: iidratio} is equivalent to at least one bidder having a value larger than $\mr$. It allows us to apply $\Lowerboundone\left (\cdot\right )$ from Lemma~\ref{lem: ziyong}. Furthermore, since the value distributions are identical, we have $\sum_{i = 1}^n\Quani(\mr) = n\cdot \Quan(\mr) = \frac{1}{\kk}$.
For $u\in[\kk, 1]$, the event $\Payment' \ge \Quan^{-1}(\frac{1}{n\cdot u})$ is equivalent to at least two bidders having values at least $\Quan^{-1}(\frac{1}{n\cdot u})$. It allows us to to apply $\Lowerboundtwo\left (\cdot\right )$ from Lemma~\ref{lem: ziyong}, where the sum of the quantiles is $\frac{1}{u}$.
I.e., we can write

\[
\frac{\Ex[\vals\sim\dists]{\Rev(\vals)}}{\opt} \ge \kk\cdot \Lowerboundone\left (\frac{1}{\kk}\right ) + \int_\kk^1\Lowerboundtwo\left (\frac{1}{u}\right )\d u
\ge \min_{\beta\in[0, 1]}\left\{\beta\cdot \Lowerboundone\left (\frac{1}{\beta}\right ) + \int_\beta^1\Lowerboundtwo\left (\frac{1}{u}\right )\d u\right\},
\]
which can be computed numerically to find the worst $\beta$, as well as the worst reserve price. Figure~\ref{fig: proof} (a) shows the curve of $\Lowerboundone\left (\frac{1}{\beta}\right )$ and $\Lowerboundtwo\left (\frac{1}{\beta}\right )$. Figure~\ref{fig: proof} (b) shows the ratio with respect to $\beta$.
The maximum ratio of $2.63$ is achieved for $\beta = \frac{1}{3}$. Thus we complete the proof for the regular margins.
\begin{figure}[htbp]
\centering  
\subfigure[Quantile bounds]{   
\begin{minipage}{7cm}
\centering    
\includegraphics[scale=0.4]{fig/Figure_1.png}  
\end{minipage}
}
\subfigure[Ratio]{ 
\begin{minipage}{7cm}
\centering    
\includegraphics[scale=0.4]{fig/Figure_2.png}%
\end{minipage}
}
\caption{Curves in the proof of Theorem \ref{thm: myersoniid}}   
\label{fig: proof}
\end{figure}
\end{proof}

For non-regular distributions, it can be shown that the revenue of mutually and pairwise independent cases is the same as that of the ironed margin. Thus it is a direct corollary of the regular case. A more specific proof is deferred to Appendix~\ref{app: non-regular}.
%\nick{TODO: Irregular distribution}

==> sec/prelim.tex <==
\begin{enumerate}
\item Conventions:
\begin{itemize}
    \item Vectors in boldface script
    \item Probability $\prob[\vals\sim\dists]{\max_{i\in[n]}\vali\ge r}$ or (macro \verb+\prob[]{},Prlong[]{}+)
    $$\Prlong[\vals\sim\dists]{\sum\limits_{i=1}^{n}\vali\ge r}$$
    \item Expectation  (macro \verb+\Ex[\vals]{\max_i \vali},\Exlong[\vals]{\max_i \vali}+)
    $$\Ex[sdf]{\max_i \vali},\Exlong[\vals]{\max_i \vali}$$
    \item Distributions in mathcal script, e.g.,  (macro \verb+\dist,\disti,\dists,\distsmi+)
    $$\dist,\disti,\dists=\prod_{i=1}^n \disti,\distsmi$$
\end{itemize}
\item Myerson auction
\begin{itemize}
    \item values $\vals=(\vali)_{i=1}^{n},\valsmi$ (macro \verb+\vali,\vals,\valsmi+)
    \item Auxiliary notations: $\valo$, $\ww$ (\verb+\valo,\ww+) 
    \item bids $\bids=(\bidi)_{i=1}^{n},\bidsmi$ (macro \verb+\bidi,\bids,\bidsmi+)
    \item allocations $\allocs=(\alloci)_{i=1}^{n}$
    (macro \verb+\allocs,\alloci+)
    \item payments $\pays=(\payi)_{i=1}^{n}$
    (macro \verb+\pays,\payi+)
    \item Total payment $\Payment$ (macro \verb+\Payment+)
    \item utility $\utili(\vali,\bidi,\bidsmi)=\vali\cdot\alloci(\bidi,\bidsmi)-\payi(\bidi,\bidsmi)$ (macro \verb+\utili+)
    \item Virtual value $\virt,\virts,\virtiri,\virti,\virtsmi$ (macro \verb+\virt,\virts,\virtiri,\virti,\virtsmi+)
    \item Maximum virtual value $\maxvirt(\vals)$ (macro \verb+\maxvirt(\vals) +)
    \item reserve $\reserve$ (macro \verb+\reserve+)
\end{itemize}
\item Lower bounds
\begin{itemize}
    \item $\Lowerboundone, \Lowerboundtwo, \Lowerboundthree$ (macro \verb+\Lowerboundone, \Lowerboundtwo, \Lowerboundthree+)
\end{itemize}
\item Distributions
\begin{itemize}
    \item Equal revenue distribution: $\ER$ (macro \verb+\ER+)
    \item Independent distribution: $\distind$ (macro \verb+\distind+)
    \item Pairwise independent distribution: $\distpi$ (macro \verb+\distpi+)
\end{itemize}
\item Quantiles
\begin{itemize}
    \item Independent quantiles: $\Qoneind, \Qtwoind$ (macro \verb+\Qoneind, \Qtwoind+)
    \item Pairwise independent quantiles: $\Qone, \Qtwo$ (macro \verb+\Qone, \Qtwo+)
    \item others $\Quan, \Quani, \Quanj$ (macro \verb+\Quan, \Quani, \Quanj+)
\end{itemize}
\item Others
\begin{itemize}
    \item moments $\momone, \momtwo$ (macro \verb+\momone, \momtwo+)
    \item tail and core $\tailrev, \corerev$ (macro \verb+\tailrev, \corerev+)
    \item used in the iid case $\kk$ (macro \verb+\kk+)
    \item $\ww, \pp$ (macro \verb+\ww, \pp+ )
\end{itemize}
\end{enumerate}

==> sec/reg.tex <==
Denote the reserve price $\reserve$, pairwise independent revenue: $\AR(\reserve)$, independent revenue: $\AR^{ind}(\reserve)$. 
\begin{lemma}[\cite{cesa2014regret}]
\label{lem: ar_revenue}
\begin{align*}
\\AR(\reserve) &= \reserve\cdot \Qone(\reserve) + \int_{\reserve}^{+\infty}\Qtwo(x)\d x,\\
\AR^{ind}(\reserve) &= \reserve\cdot \Qoneind(\reserve) + \int_{\reserve}^{+\infty}\Qtwoind(x)\d x.    
\end{align*}
\end{lemma}

Denote $\payi = \Quani(1)$.
\begin{lemma}
\label{lem: reg_quantile}
$\forall \val\geq 1,$ we have
\begin{equation*}
\Quani(\val) \leq \frac{\payi}{(1 - \payi)\cdot \val + \payi}.
\end{equation*}
$\forall \val\leq 1,$ we have
\begin{equation*}
\Quani(\val) \geq \frac{\payi}{(1 - \payi)\cdot \val + \payi}.
\end{equation*}
\end{lemma}
\begin{proof}
The revenue is larger than 0 when the quantile is 1. The revenue is $\payi$ when the quantile is $\payi$.
According to the regularity (see fig. \ref{fig: reg_curve}), for $\val\geq 1$ we have
\begin{equation*}
    \val\cdot \Quani(\val)\leq -\frac{\payi}{1 - \payi}\cdot \Quani(\val) + \frac{\payi}{1 - \payi}.
\end{equation*}
For $\val\leq 1$ we have
\begin{equation*}
    \val\cdot \Quani(\val)\geq -\frac{\payi}{1 - \payi}\cdot \Quani(\val) + \frac{\payi}{1 - \payi}.
\end{equation*}
Simple math manipulation leads to the conclusion.
\begin{figure}
\centering
    \includegraphics[width=8cm]{fig/regular.png}
    \caption{Regular revenue curve}
    \label{fig: reg_curve}
\end{figure}
\end{proof}

\begin{proposition}
\label{pro: convex}
It is easy to verify that:
\begin{equation*}
\frac{\d^2 }{\d x^2}\frac{x}{(1 - x)\val + x} = \frac{2\val(\val - 1)}{\val - (\val - 1)x}.  
\end{equation*}
Thus for $x\leq 1$, it is concave when $\val\leq 1$ and it is convex when $\val\geq 1$.
\end{proposition}

==> sec/related.tex <==
\nick{TODO: edit this section}

%%%% Single-item auction: robust mechanism for correlated prior, computational results, simple vs. optimal
The body of work on revenue maximization in single-item auctions is too large to describe within the scope of our paper. We mention a few papers that are most closely related to our setting.
% There has been a lot of work dedicated to the revenue maximization in single-item auctions, which is too much to overview within the scope of our paper. 
For the case of correlated 
prior $\dists$ Bei et al.~\cite{BeiGLT19} and He and Li~\cite{HeL22} identify (approximately) optimal mechanism within the correlation-robust framework, i.e., mechanisms that are given marginal distributions $(\disti)_{i\in[n]}$ but are unaware of the correlation structure.
On the computational side, Papadimitriou and Pierrakos~\cite{papadimitriou2011optimal} proved NP-hardness of finding revenue optimal mechanism under ex-post individual rationality constraint, while Dobzinski et al.~\cite{dobzinski2011optimal} showed that optimal 
randomized mechanism can be found polynomial in the prior's support size, and a simple and approximately optimal lookahead auction by Ronen and Saberi~\cite{RonenS02} is easy to compute. When the prior $\distind$ is independent, a few papers give multiple approximation guarantees on the revenue of simple auction formats such as sequential posted-pricing, second-price auction with an anonymous reserve, anonymous pricing, and second-price auction with monopoly reserves to the optimal revenue of Myerson's auction~\cite{CorreaSZ19,DuttingFK16,HartlineR09,jin2020tight}.

There are many other settings that have been studied within the purview of robust mechanism design. For example monopoly problem with a single-item~\cite{CarrascoFKMMM18}, an additive buyer~\cite{carroll2017robustness,GravinL18}, and a unit-demand buyer~\cite{BabaioffFGLT20}; contract design, e.g.,~\cite{carroll2015robustness,carroll2016robust,DuttingRT19}; multi-item auctions~\cite{BandiB14}.

\wzq{In a recent paper \cite{dughmi2023limitations}, the authors show that both prophet inequality and contention resolution cannot achieve a constant balance or competitive ratio in the worst pairwise independent distribution.}

%%%%% Pairwise-independence
The setting most closely related to ours is studied by Caragiannis et al.~\cite{caragiannis2022relaxing}. They consider multiple approximation 
results on prophet inequality, sequential posted pricing, and random bipartite matching
for the mutually independent distribution $\distind$ and show that these results can be extended to any pairwise independent distribution $\dists\in\distpwi$ at an additional small  multiplicative factor. In particular, their results imply that a variant of sequential posted pricing for single-item auctions is pairwise-robust. They also mention that the analysis of 
Babaioff et al.~\cite{BabaioffILW20} for the monopolist problem with additive buyer gives a stronger guarantee that the respective simple mechanism is pairwise-robust.  

%%% Discussion about max-min optimal mechanism
\paragraph{Comparison to Robust Mechanism Design.}
Our model falls under the umbrella of robust mechanism design, which has received significant attention in recent years (see e.g.,~\cite{BabaioffFGLT20,BandiB14,BeiGLT19,bergemann2011robust,caragiannis2022relaxing,carroll2015robustness,carroll2016robust,DuttingRT19,garrett2014robustness,GravinL18}). 
This line of work generally relies on a robust optimization framework, tracing back to the classic work in Operation Research by Scarf~\cite{Scarf1958minmax}. I.e., the objective is to optimize the mechanism's expected performance in the worst case across all prior distributions with a given partial information about the prior. The typical goal of this research agenda is to identify the optimal min-max mechanism. Conversely, we deliberately use constant approximation as the criterion for separating robust mechanisms from non-robust mechanisms.
Indeed, the min-max solution is pessimistic by its very nature and thus not likely will be used as the dominant criterion for choosing the mechanism/auction format. 
Furthermore, even in a basic setting of single-item auctions, one can consider many reasonable information structures for the min-max optimization that likely would lead to very different optimal auction formats. 
Our pairwise-robust information structure $\distpwi$, on the one hand, is much closer to the fully known prior $\dists=\prod_{i\in[n]}\disti$ than almost all other information structures considered in the previous work. On the other hand, it already allows one to separate the optimal Myerson's mechanism from certain simple mechanisms such as second-price auction with an anonymous reserve and sequential posted pricing (it was shown to be pairwise-robust 
by Caragiannis et al.~\cite{caragiannis2022relaxing}) and show their unbounded potential advantage over more complex Myerson's mechanism. 



 

% Most of the work on Bayesian single-item auction for general (correlated) prior distribution concerns the optimal auction design with respect to a given prior.
% It was shown in~\cite{CremerMcLean85} that full social surplus can be extracted if the joint prior distribution is generic in a certain sense.
% % Their result was extended in~\cite{McAfeeReny92} to continues type spaces, and by~\cite{Genericity13} to generic prior distributions in a properly
% % defined topological space over the set of all prior distributions. 
% From a computational perspective, it was shown in~\cite{papadimitriou2011optimal} that computing the optimal
% mechanism under ex-post individual rationality constraint is NP-hard. On the other hand, for randomized mechanisms~\cite{dobzinski2011optimal} showed that optimum can be
% computed in time polynomial in the size of the distribution's support.

%%%% Robust mechanisms in other settings: computational results 








% Assuming the bidders' value are mutually independent, the seller can implement Myerson auction to achieve the optimal revenue \cite{myerson1981optimal}. However, from the statistics point of view, it would be hard to test whether a group of random variables are mutually independent. It will suffer from the curse of dimension thus a weaker notion of independence is required. 

% Carroll proposes the scheme of correlation robust mechanism: suppose the mechanism designer only knows the marginal distribution of the random variables, trying to design a mechanism which performs optimal in the worst joint distribution \cite{carroll2017robustness}. The author considered the multidimensional screening problem and proved that selling separately is optimal. Gravin and Lu further extended the result to budget constrained buyers \cite{gravin2018separation}.

% Note that the correlation robust mechanism scheme makes no assumption on the joint distribution. In a recent paper, Caragiannis \etal considered the robustness of pairwise independent random variables and proved that several mechanisms can achieve a constant ratio compared with their performance in the independent case.
% Inspired by their results, we propose the definition of pairwise independence robust auction:

==> sec/techniques.tex <==
Similar to Caragiannis et al.~\cite{caragiannis2022relaxing} we consider the integral representation of revenue as the payment of the respective auction. However, in their work,  Caragiannis et al. only need to analyze simple events $E_1(\tau)$ that at least one bidder exceeds a threshold $\tau$, while second price auction with anonymous reserve requires us to consider events $E_2(\tau)$ that at least two bidders are above the threshold $\tau$. 
Handling the latter events poses a significantly bigger challenge than the former within the pairwise-independent framework. Indeed, Caragiannis et al. can directly prove a constant factor gap between probabilities in mutually and pairwise independent cases for all events $E_1(\tau)$. Such constant factor gap no longer holds for to $E_2(\tau)$ events. We have to actively use the fact that distributions are regular and carefully compare different parts of respective integral representations for mutually independent and pairwise independent priors.

We also have to find an example showing that Myerson's auction is not pairwise-robust. The example is not very complex, but also rather non-trivial. It was frankly quite surprising to us, given that for the case of identical marginals $\disti=\dist$ Myerson's auction is pairwise-robust.

% \paragraph{Regularity Assumption for Marginals.}
% Throughout this paper we always assume that all marginal distributions  
% $(\disti)_{i\in[n]}$ are regular. As we mentioned before, one reason for not considering irregular priors is that the revenue gap between Myerson's mechanism and AR may be arbitrary large. Another reason is that Myerson's mechanism is not unique for irregular marginals. To illustrate this point, consider the case of identical irregular marginals $\disti=\dist$. In this case $\dist$ has to be ironed at least somewhere, e.g., on an interval $[a,b]$ above the monopoly reserve. Then all bidders with values $\vali\in[a,b]$ have the same virtual values. Hence, there is a non zero chance that Myerson's mechanism will need to break ties to pick one of the bidders in the interval $[a,b]$. There are many ways it can break ties, e.g., uniformly at random, or lexicographically. Moreover, if the distribution $\dist$ is regular with an ironed interval $[a,b]$, e.g., equal revenue distribution, then optimal mechanism may use bidders' values to break ties (for example, SPA with monopoly reserve is an optimal mechanism in this case). The non uniqueness of Myerson's mechanism is not a problem for the mutually independent prior $\distind$, but it may lead to different revenues on different pairwise-independent priors $\dists\in\distpwi$.

  
% All our results are only for the case of regular marginals
% $(\disti)_{i\in[n]}$

% Interestingly, for the case of irregular marginals $(\disti)_{i\in[n]}$ the Myerson's mechanism is not unique. To illustrate this, consider the case of identical priors 
